Towards Efficient and Scalable Sharpness-Aware Minimization

Recently, Sharpness-Aware Minimization (SAM), which connects the geometry of the loss landscape and generalization, has demonstrated significant performance boosts on training large-scale models such as vision transformers. However, the update rule of SAM requires two sequential (non-parallelizable) gradient computations at each step, which can double the computational overhead. In this paper, we propose a novel algorithm LookSAM - that only periodically calculates the inner gradient ascent, to significantly reduce the additional training cost of SAM. The empirical results illustrate that LookSAM achieves similar accuracy gains to SAM while being tremendously faster - it enjoys comparable computational complexity with first-order optimizers such as SGD or Adam. To further evaluate the performance and scalability of LookSAM, we incorporate a layer-wise modification and perform experiments in the large-batch training scenario, which is more prone to converge to sharp local minima. We are the first to successfully scale up the batch size when training Vision Transformers (ViTs). With a 64k batch size, we are able to train ViTs from scratch in minutes while maintaining competitive performance.

==> fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\columnwidth]{example-image-golden}
\hfill
\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Outline -- }
A figure summarizing the entire algorithm
}
\label{fig:overview}
\end{figure*}

==> tab/ablations.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Ours v0 & Frumpy \\
Ours v1 & Frobbly \\
\textbf{Ours} & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
\textbf{Ablations} -- our decisions are well justified.
% 
} % \caption
\label{tab:ablations}
\end{table}

==> tab/acc_cifar10.tex <==
\begin{table*}[ht]
\renewcommand\arraystretch{1.2}
\caption{Accuracy of different Models on CIFAR10 \color{blue}{(Need to update and add some description)}}
\label{tab_cifar10}
\begin{center}
\begin{tabular}{l|c|cc|cc|cc|c}
\multicolumn{1}{c|}{\bf Model} &\multicolumn{1}{c|}{\bf AdamW}
&\multicolumn{1}{c}{\bf SAM-5}
&\multicolumn{1}{c|}{\bf LookSAM-5}
&\multicolumn{1}{c}{\bf SAM-10}
&\multicolumn{1}{c|}{\bf LookSAM-10} 
&\multicolumn{1}{c}{\bf SAM-20}
&\multicolumn{1}{c|}{\bf LookSAM-20}
&\multicolumn{1}{c}{\bf SAM} 
\\ \hline
\multicolumn{1}{l|}{\bf WRN-28-10}       &  96.5    & 97.2 & \textbf{97.3} & 97.0  & \textbf{97.1} & 96.8 & \textbf{97.0} & 97.3\\

% WRN-28-2       &   &  & \\
\multicolumn{1}{l|}{\bf ResNet-18}       & 95.6   & 96.2 &96.2 &96.0  & \textbf{96.1} &96.0 &\textbf{96.1} & 96.4 \\
\multicolumn{1}{l|}{\bf ResNet-50}       & 95.7   & 96.6 & \textbf{96.8} & 96.5  & \textbf{96.6} &96.2 & \textbf{96.4} &96.9 \\

\hline
\end{tabular}
\end{center}
\end{table*}


==> tab/sota.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
% 
\textbf{State of the art} -- Glory to the bold numbers.
% 
} % \caption
\label{tab:sota}
\end{table}
